Planning, Fast and Slow: A Framework for Adaptive Real-Time Safe Trajectory Planning

Motion planning is an extremely well-studied problem in the robotics community, yet existing work largely falls into one of two categories: computationally efficient but with few if any safety guarantees, or able to give stronger guarantees but at high computational cost. This work builds on a recent development called FaSTrack in which a slow offline computation provides a modular safety guarantee for a faster online planner. We introduce the notion of "meta-planning" in which a refined offline computation enables safe switching between different online planners. This provides autonomous systems with the ability to adapt motion plans to a priori unknown environments in real-time as sensor measurements detect new obstacles, and the flexibility to maneuver differently in the presence of obstacles than they would in free space, all while maintaining a strict safety guarantee. We demonstrate the meta-planning algorithm both in simulation and in hardware using a small Crazyflie 2.0 quadrotor.

==> pseudocode.tex <==
\begin{algorithm}
	\SetKwIF{Wp}{WpElseIf}{WpElse}{with probability}{do}{else if}{otherwise}{}
	\KwIn{$x_{\text{start}},\;
			x_{\text{goal}},\;
			\pi_1, ..., \pi_K,\;\\
			\mathcal{E}_1, ..., \mathcal{E}_K,\;
			\mathcal{E}_{1 \to 2}, ..., \mathcal{E}_{(K-1) \to K}$}
	\KwOut{tree,$\;$plan}
	\BlankLine
	\textbf{Initialization}\DontPrintSemicolon\;\PrintSemicolon
		tree.root.x 		$\gets x_\text{start}$\;
		tree.root.k 		$\gets K$\;	% max k for trivial expansion (without transition)
		tree.root.g 		$\gets 0$\;
		tree.root.h 		$\gets h_1(x_{start},x_{goal}))$\;
		\BlankLine
	\textbf{Tree Expansion}\DontPrintSemicolon\;\PrintSemicolon
		\While{not done}{
			\uWp{increasing in n\_orphans}{
				candidate $\gets$ tree.orphans.extractFirst( )\tcp*{orphan with best heuristic}
			}
			\WpElse{
				candidate $\gets$ sample\_from\_free\_space( )\tcp*{e.g. Informed RRT*}
			}
			closest\_node $\gets \displaystyle\arg\min_{\text{node}\in\text{tree}} h_1(\text{node.x},\text{candidate.x})$\;
			$k\gets 0$\;
			(success, hope, switchable) $\gets$ false\;
			\While(\tcp*[f]{try planners fast $\to$ slow}){not success \textbf{and} not hope \textbf{and} $k<K$} {
				$k\gets k+1$\;
				success $\gets$ collision\_free(closest\_node.x, candidate.x, $\mathcal{E}_{k}$)\;
				\If(\tcp*[f]{verify planner switch}){$k > \text{closest\_node.k}$ \textbf{and} success}{
					hope $\gets$ success\;
					switchable $\gets$ collision\_free(closest\_node.x, candidate.x, $\mathcal{E}_{(k-1)\to k}$)\; % NOTE: assuming cost_j = cost_{i->j}
					success $\gets$ switchable \textbf{and} ($k$$-$1 == \text{closest\_node.k})
				}
			}
			\uIf{success}{
				candidate.g $\gets$ closest\_node.g + get\_cost(closest\_node.x, candidate.x, $\pi_k$)\;
				closest\_node.addChild(candidate)\tcp*{add new node to tree}
			}
			\ElseIf{hope}{
				k\_need $\gets k - 1 \times$(switchable)\;
				% check if backtrack node already exists as sibiling
				\If{closest\_node.parent.hasChild(x=closest\_node.x,k=k\_need)}{
					closest\_node.parent.getChild(\\x=closest\_node.x,k=k\_need).addChild(candidate)\;
				}
				\Else{
					backtrack\_node.x $\gets$ closest\_node.x\;
					backtrack\_node.h $\gets$ closest\_node.h\;	% g will be assigned at adoption
					backtrack\_node.k $\gets$ k\_need \;
					tree.orphans.insertSortedBy(backtrack\_node, $h_1(\text{self.x},x_\text{goal})$)\tcp*{add orphan to tree}
				}
			}%\ElseIf{hope}
		}%While{not done}
		plan $\gets$
		$\big($
		$\displaystyle\arg\min_{\text{node}\in\text{tree}|\text{node.x}=x_\text{goal}}$
		$\text{node.g}$
		$\big)$\text{.tree\_path\_to()}
\caption{Meta-planning with Backtracking\label{alg:backtrack}}
\end{algorithm}
